Machine Unlearning of Pre-trained Large Language Models

This study investigates the concept of the `right to be forgotten' within the context of large language models (LLMs). We explore machine unlearning as a pivotal solution, with a focus on pre-trained models--a notably under-researched area. Our research delineates a comprehensive framework for machine unlearning in pre-trained LLMs, encompassing a critical analysis of seven diverse unlearning methods. Through rigorous evaluation using curated datasets from arXiv, books, and GitHub, we establish a robust benchmark for unlearning performance, demonstrating that these methods are over $10^5$ times more computationally efficient than retraining. Our results show that integrating gradient ascent with gradient descent on in-distribution data improves hyperparameter robustness. We also provide detailed guidelines for efficient hyperparameter tuning in the unlearning process. Our findings advance the discourse on ethical AI practices, offering substantive insights into the mechanics of machine unlearning for pre-trained LLMs and underscoring the potential for responsible AI development.

==> o2-formulation.tex <==
% \du{I) Incorporate ``adaptive'' unlearning~\cite{nips/GuptaJNRSW21}?; adaptivity here means that the token sequences to be unlearnt can be chosen based on the prior ``outputs.'' 
% II) lost in current formulation; I understand our current goal is trying to ``generalize'' the existing definitions (like $(\epsilon, \delta)$-unlearning~\cite{nips/SekhariAKS21}).
% But, it turns out that the formulation falls inside $(\epsilon, \delta)$-unlearning, as we still focus on ``characterizing $\mathcal{U}$,'' which essentially can be captured by the sequences to be unlearnt: the set of adaptively-chosen sequences define a type of ``harmful'' behavior. 
% In short, why re-invent the wheel (if without big differences)?
% }
\eli{For I) sure I can try to incorporate that. For II), our type I unlearning is indeed the same as $(\epsilon, \delta)$-unlearning, which is the most natural thing for privacy applications. However, for type II unlearning it becomes very different. The key here is that type I unlearning is defined by "the effect of which training sequences to be removed". On the other hand, type II unlearning is defined as "preventing the output from being harmful/undesired behavior". Note that an undesired behavior may not be the effect of a single or subset training sequence, it can be a complex implication of all training sequences. see the example in section 2.3 for example. Still, it's good that Minxin asks this question, as now I feel type II unlearning may be relevant to unlearning a class in classification.}
\du{thx! I can also take responsibility for this part (but the first thing is to let me figure out what can I do based on prior arts and what we have done).}
\xy{It is similar to unlearning a class at the high level, but our Type II scenario is indeed much more complex. First, it is hard to define a real ``class'' here. Secondly, again, we are not unlearning training samples here.}
\du{For 2nd point, I think we are still unlearning \emph{training examples} defining a behavior/class; otherwise, it's not suitable to call it unlearning?}
%\du{Some other context/bground: Harry potter one first uses reinforced model to identify related terms (to be forgotten), making me ``link'' it to using NER to tag PII.}


\textbf{Behavioral Unlearning. }We now introduce the concept of our novel behavioral unlearning in the language modeling setting. The goal of behavioral unlearning is to efficiently update $M$ to $M^\prime$ after we receive some behavioral regulations defined by $\mathcal{U}$. 
% \du{Comments on Eq.~(2): 
% i) $\mathcal{U}$ is not explicitly defined. 
% Not suitable to view it as ``behavioral regulations,'' not comparable with $P_{M^\prime}$, a probability distribution.
% So, $\mathcal{U}$ should also be a probability distribution (of the unlearnt model).
% ii) For $\mathcal{L}(P_{M^\prime};\mathcal{D})$, it should be something like $\mathcal{L}(P_{M^\prime};\mathcal{D} \setminus S)$, where $S$ is the set of sequences to be removed.}
Conceptually, this is equivalent to achieving the objective below starting with $M$:
\begin{align}\label{eq:behavioral_unlearn}
    \min_{M^\prime} \mathcal{L}(P_{M^\prime};\mathcal{D}) \text {  subject to  } d(P_{M^\prime};\mathcal{U})\leq \xi,
\end{align}
where $d(P_M;\mathcal{U})$ measures how severely $M$ violates behavioral regulations and $\xi$ is the slackness of the violations that we would tolerate. We would like to emphasize that while retraining from scratch can resolve~\eqref{eq:behavioral_unlearn}, it is prohibitively expensive in time and cost for LLM, e.g., consuming weeks to months of computation on high-end GPUs, costing millions of dollars, and producing a significant amount of carbon footprint~\cite{corr/LuccioniVL22}.

% \eli{To Tianhao's questions: for privacy, simple retraining can obviously satisfy it, since we will know which node to be unlearned from $\mathcal{U}$. For other applications, take fairness as an example. There are many ML techniques that can ensure the model satisfies fairness constraints (provided by $\mathcal{U}$). It is also straightforward to remove outdated information, where retraining without outdated samples can achieve our goal.}

% We assume the LLM service provider will always keep their LLM $M$ private. Any user can interact with $M$ potentially infinitely many times, which is equivalent to accessing the model output distribution $P_{M}(w_{t+1} | w_1, w_2, ..., w_t)$ for any input $(w_1, w_2, ..., w_t)$. \eli{Maybe explain why this assumption is practical.} 

Comparing individual weights or parameters of LLMs directly can be computationally challenging and may not provide a clear understanding of practical differences due to their massive amount of parameters. A more insightful approach is to assess how unlearning influences the model's behavior. This can be achieved by gauging the output distributions, offering an immediate insight into the model's behavioral modifications. In practical terms, the utility of $M$ (i.e., downstream performance) or any potential violations of behavioral regulations can predominantly be inferred from its output distribution $P_M$. Our behavioral unlearning problem is general. It covers applications ranging from safeguarding data privacy, mitigating copyright infringement, eliminating outdated and incorrect information, addressing harmful and biased narratives, and customized model deployment. Each application corresponds to different definitions of regulations $\mathcal{U}$ and the measure of violation $d$. 

Safeguarding data privacy is the main focus of the general machine unlearning literature, which is more well-understood compared to the other applications. Nonetheless, it is crucial to recognize that the principles and methodologies of machine unlearning can be applied to numerous other domains, transcending the scope of privacy, and this broader applicability holds significant practical value. Our comprehensive conceptualization of behavioral unlearning illuminates the growing spectrum of applications that extend beyond the realm of privacy. Below we discuss two representative applications of behavioral unlearning: safeguarding data privacy and addressing harmful and biased narratives. Our primary focus is on the characterization of $\mathcal{U}$ and $d$, their similarities and differences for the two applications. A more thorough discussion of the other applications is postponed to Section~\ref{}. 

% \eli{To everyone: can check if above sounds better than our previous story.} \xy{Thanks. I revised it a little bit and added additional transition sentences to make it more coherent. I'm thinking whether we would like to actually introduce this new term ``behavioral unlearning'' or just say we extend the original unlearning definition to a more broad way. } \eli{LGTM.}

\subsection{Unlearning for ``Right-to-be-forgotten (RTBF)''}
\label{sec:BU_privacy}


% With the adoption of recent laws ensuring the “right to be forgotten”, the problem of removing the effect of some training data from $M$ has become of significant importance. Machine unlearning was initially proposed for this privacy application and has become imperative due to privacy regulations, including the European Union’s General Data Protection Regulation (GDPR), the California Consumer Privacy Act (CCPA), and the Canadian Consumer Privacy Protection Act (CPPA). Theoretical machine unlearning researches~\cite{icml/GuoGHM20,nips/SekhariAKS21,iclr/Chien0M23} define privacy by comparing the distribution of obtaining $M^\prime$ and $M$. However, since most LLMs subject to privacy concerns are kept private and only allow access to their output, their privacy definition can be too pessimistic. Instead, it is sufficient to protect privacy protection by comparing the model output distribution $P_M$ and $P_{M^\prime}$, which is also related to the setting of prediction differential privacy~\cite{}\eli{To Tianhao: could you recommend several references along this line?}. 

Consider a scenario in which multiple data sequences $x_i$ are requested for removal in accordance with the right to be forgotten. $\mathcal{U}$ are set to be the subset $\mathcal{U}\subseteq \mathcal{D}$ subjected to data sequences to be forgotten. The gold standard for removing the effect of $\mathcal{U}$ is to retrain from scratch on $\mathcal{D} \setminus \mathcal{U}$,
%$\mathcal{D}\subset \mathcal{U}$, 
where we denote such retrained model as $M^{\mathcal{U}}_r$. ``Closer'' $P_M$ and $P_{M^\mathcal{U}}$ leads to less privacy leakage. There are several choices of $d$ for this measure. For instance, one can adopt the formulation of R{\'e}nyi differential privacy~\cite{csfw/Mironov17} related to prior theoretical unlearning researches~\cite{icml/GuoGHM20,nips/SekhariAKS21,iclr/Chien0M23}.
\begin{align}\label{eq:rdp_unlearning}
    & \sup\left(D_{\alpha}(P_{M^\prime}||P_{M^{\mathcal{U}}_r}),D_{\alpha}(P_{M^{\mathcal{U}}_r}||P_{M^\prime})\right)\leq \xi,
\end{align}
where $D_{\alpha}$ is the R{\'e}nyi divergence of order alpha and the supremum is also taken over all possible model input-output pairs. While other probability ``distance'' measures can be adopted as we will introduce later, the specific choice of Eq.~\ref{eq:rdp_unlearning} can be strongly related to the error rate of the optimal hypothesis testing on distinguishing $P_M$ from $P_{M^\prime}$~\cite{icml/KairouzOV15,googleunlearning}. In other words, if we achieve the case of $\xi=0$, it is fundamentally impossible for \emph{any} adversary to infer with confidence if they are interacting with $M^\prime$ or $M_r^{\mathcal{U}}$. As a result, the information pertaining to data sequence in $\mathcal{U}$ is hidden and thus their privacy is protected.\eli{Maybe Tiahao or Minxin can provide some other better refs? I also intend to make the last few sentences vague but easy to understand. I know rigorously speaking we should measure the probability of having $P_M$, but I think it is unrealistic and too technical. Still, please let me know if they are incorrect.}
In practice, enumerating all possible input-output pairs is impossible. Researchers working on machine unlearning for deep neural networks proposed comparing $P_M$ and $P_{M^\prime}$ only on the $\mathcal{D}$, $\mathcal{U}$ or $\mathcal{D}\setminus\mathcal{U}$. Choices other than R{\'e}nyi divergence are also considered, such as difference in classification (downstream) accuracy~\cite{cvpr/GolatkarAS20,nips/JiaLRYLLSL23}\eli{add more} and Jensen-Shannon divergence~\cite{tit/Lin91,aaai/ChundawatTMK23}.

\subsection{Unlearning Beyond RTBF}\label{sec:BU_harmful}

The goal here is ensuring the unlearned LLM output $P_{M^\prime}$ satisfies the regulations described by the behavioral regulations defined by $\mathcal{U}$ directly. \eli{We might want to give a concrete formulation here. Even a simple case is fine. Maybe we can have a brainstorm for this part. Below I just give a naive example.}. Consider the case where $\mathcal{U}=\{u_j=(w^j_{t+1}|w^j_{t},\ldots,w^j_{1})\}$ defines a set of input-output pairs that are subject to harmful and biased narratives. The goal would be to ensure that $\forall u\in\mathcal{U},\; P_{M^\prime}(u)\leq \xi$. As a result, the violation measure $d$ would be
\begin{align}
    \sup_{u\in \mathcal{U}} P_{M^\prime}(u).
\end{align}
Apparently, there are other designs of $\mathcal{U},d$, and the most appropriate choice of $\mathcal{U},d$ for each application other than privacy is under-explored in the literature. We encourage the collaboration of experts from trustworthy AI, LLM, and machine unlearning domains for designing the proper definitions and the corresponding unlearning techniques. 

\subsection{Behavioral Unlearning for General Tasks}\label{sec:BU_general}
Notably, there are two types of behavioral regulations under the umbrella of our behavioral unlearning: one is defined by {\it comparing with retraining} as discussed in Section~\ref{sec:BU_privacy}, and the other one is defined by {\it direction constraints} on the model output distribution without comparison to retraining as discussed in Section~\ref{sec:BU_harmful}. We denote them as \textbf{type I} and \textbf{type II} behavioral unlearning respectively. This critical difference is the key contribution of our behavioral unlearning formulation. Whether which type of behavioral regulation we should choose depends on the goal of each application. For privacy applications, we indeed require erasing the effect of some specific data sequences from the LLM. Due to the complex nature of the LLM, it is impossible to characterize the effect of those training data sequences on the LLM explicitly other than comparing with retraining. Type I behavioral unlearning can also apply to other applications. For instance, authors of copyrighted content may request the LLM holder to unlearn the effect of that content if they have been used for training. Another example is to remove the effect of outdated, poisoned, and incorrect data effect from the LLM. However, type I behavioral unlearning is not suitable for the scenario where we have to ensure the LLM output satisfies some explicit constraints, such as fairness and not being harmful. The issue is that even if we completely remove the effect of some training sequences (i.e., sequences that directly contain harmful content), there is no guarantee that the resulting LLM would not have undesired output due to its complex nature. A potential example to illustrate this phenomenon is as follows: while concepts $A\rightarrow B$ and $B \rightarrow C$ in two distinct training sequences are not harmful individually and thus not subject to be unlearned, the LLM trained on both sequences may output the concept $A\rightarrow C$ which can actually be harmful \eli{i.e., Eli is black, Ape is black, ... I don't want to use explicit example otherwise our paper can be harmful itself lol.} \xy{That's fine. People usually add a warning on the front page. I just added.}.  

As a result, there are also scenarios where we need to ensure that LLM will not have behavior that violates some rules directly, where type II behavioral unlearning is needed. Besides the examples provided above and in Section~\ref{sec:BU_harmful}, we may also ensure the LLM not outputting copyright content, outdated or incorrect information. It is also interesting to note that for some applications, both types of behavioral regulations can apply. Thus, they are not exclusive from each other for each task. It really depends on the underlying purpose that we aim for: erasing the effect of some training sequences or ensuring LLM output regulations. It is also possible to require both simultaneously if necessary.


% Examples include preventing the LLM from producing outdated and incorrect answers, or harmful and biased narratives. In this case, the unlearning request $\mathcal{U}$ is not a subset of training samples, but a set of regulations and constraints on the LLM output distribution $P_{M}$. The most critical difference between training data and behavioral unlearning is that the former set ``regulations'' on training input while the latter directly regularize the model output $P_{M}$. An immediate result of this key difference is that we do not need to compare with retraining from scratch model $M_r^{\mathcal{U}}$ for behavioral unlearning. We can simply check if $P_{M^{\mathcal{U}}}$ satisfy the regulations pertaining to $\mathcal{U}$, which also makes the evaluation more practical. \eli{We might want to add a figure to illustrate training data v.s. behavioral unlearning.} \xy{I'm thinking about it as well. I could try to plot one once we get a better text version.}

% While the difference between training data and behavioral unlearning may seem subtle, we note that they are suitable for different applications and cannot be replaced by each other. Take user data privacy as an example. Forcing $P_{M^{\mathcal{U}}}$ to be similar to any reference output distribution other than $P_{M_r^{\mathcal{U}}}$ will inevitably breach the user data privacy, as $\mathcal{U}\subseteq\mathcal{D}$ can be inferred by comparing $P_{M^{\mathcal{U}}}$ with $P_{M_r^{\mathcal{U}}}$ in the worst case\tw{don't understand what you want to say} \eli{I was trying to convey the idea that the (most powerful) adversary can perform optimal hypothesis testing on the distribution (current vs retraining) to determine whether $\mathcal{U}$ is used or not. So we really need to compare with retraining in this case.}\tw{but is it related to `difference between training data and behavioral unlearning'?}. While exact output distribution may be hard to obtain for the adversary in practice, approaches such as membership inference attacks can be adopted. Furthermore, the model weight $M$ also leaks the user data privacy information if it is made public. Definition~\ref{def:eps_del_unlearning} guarantees that even under the worst scenario that $M^{\mathcal{U}}$ is released and $P_{M^{\mathcal{U}}}$ can be obtained, any adversary cannot infer information about $\mathcal{U}$ with certainty. On the other hand, let us consider the scenario where we would like to prevent LLMs from providing harmful answers. Such a harmful bias can either exist for \emph{most} of the training data or be hard to quantify which samples result in such answers due to the complex model nature. Removing the effect of a subset of samples (if we can find them) does not necessarily resolve the problem. Behavioral unlearning seeks to address and rectify these issues, which regulates the model output behavior $P_{M^{\mathcal{U}}}$ directly. This might involve techniques like fine-tuning with corrected data, using counterfactual data augmentation, or introducing regularization methods to penalize biased outputs. 
%  \tw{i feel Behavioral Unlearning is too broad. e.g., what openai does to prevent chatgpt from describing risky things can be Behavioral Unlearning?} \eli{For the goal that we want to achieve, yes. However, if openai simply uses hard rules to filter out risky contents, it might still have some risk of being "jailbroke". On the other hand, it does not provide a smooth slackness of how well we should follow these rules (like $(\epsilon,\delta)$ thing in privacy). We hope to get the model weight that naturally satisfies these constraints with a smooth control.}\tw{ok. this is interesting. perhaps acknowledge this is related to what openai is doing. i also feel similar ideas has been eluded e.g., in \cite{ndss/WarneckePWR23} (they propose to unlearn only parts of the image instead of the whole image)}

% \xy{Randomly put some stuff here.. feel free to adapt and modify}
% ``Behavioral Unlearning'' targets the broader, emergent responses or behaviors of a machine learning model, rather than focusing on specific training samples. In this scenario, the model, during its inference phase, might produce undesirable, biased, or potentially harmful outputs due to embedded flaws or biases in its parameters. These biases or flaws might not be directly traceable to explicit training samples but result from more subtle patterns the model has learned from its training data. Behavioral unlearning seeks to address and rectify these issues, ensuring that the model no longer produces such outputs. This might involve techniques like fine-tuning with corrected data, using counterfactual data augmentation, or introducing regularization methods to penalize biased outputs.

% \eli{Here we can introduce several examples of what do we mean by regulations with math formulas for different scenarios. I think we can put math formulas here and detail discussion and evaluation metrics in Section 3.} 

% \begin{table*}[!t]
% \small
% \centering
% \begin{tabular}{@{}lcc@{}}
% \toprule
% \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{Training Data Unlearning} & Behavioral Unlearning \\ \midrule
% \multicolumn{3}{c}{Unlearning Applications} \\ \midrule
% \multicolumn{1}{l|}{Mitigating copyright infringements} &  \multicolumn{1}{c|}{\mycheck} & \mycross  \\
% \multicolumn{1}{l|}{Safeguarding data privacy} & \multicolumn{1}{c|}{\mycheck} & \mycross  \\
% \multicolumn{1}{l|}{Removing outdated information} & \multicolumn{1}{c|}{\mycheck} & \mycheck  \\ 
% \multicolumn{1}{l|}{Addressing harmful and biased narratives} & \multicolumn{1}{c|}{\mycheck} & \mycheck  \\
% \multicolumn{1}{l|}{Customized model deployment} & \multicolumn{1}{c|}{\mycheck} & \mycheck  \\ \midrule
% \multicolumn{3}{c}{Unlearning Methods} \\ \midrule
% \multicolumn{1}{l|}{Retrain} & \multicolumn{1}{c|}{} &  \\
% \multicolumn{1}{l|}{Gradient ascends} & \multicolumn{1}{c|}{} &  \\
% \multicolumn{1}{l|}{Fine-tune on retain dataset} & \multicolumn{1}{c|}{} &  \\
% \multicolumn{1}{l|}{Fine-tune with reference distribution} & \multicolumn{1}{c|}{} &  \\ \bottomrule
% \end{tabular}%
% \caption{Summary of unlearning applications and methods in the two settings. \mycheck~and~\mycross~means whether the application/method is applicable to the corresponding setting. }
% \label{tab:}
% \end{table*}


% \section{Applications}
% In this section, we will discuss some typical scenarios where unlearning plays a significant role in addressing potential concerns. For each application, we will start by introducing the scenario, followed by formal formulation and evaluation metrics. \tw{i feel those are somewhat hinted already in sec 2.1 and 2.2. somehow merge them into sec 2.1 and 2.2?}

% \paragraph{Mitigating copyright infringements.}
% LLMs have the potential to internalize and reproduce copyrighted content unintentionally. This poses not only legal challenges but also ethical dilemmas, particularly when the model's outputs mimic or rephrase the protected material. When it comes to light that copyrighted data has been assimilated into an LLM's training set, machine unlearning techniques can be used to facilitate the model's ``forgetfulness'' regarding this specific content. By doing so, the model's subsequent outputs are safeguarded against undue influences of the copyrighted material, fostering a more compliant and ethical use of data.

% \paragraph{Safeguarding data privacy.}
% The immense and eclectic datasets that LLMs are trained on carry the risk of embedding personally identifiable information (PII) or other sensitive user details. In situations where an LLM is found to have internalized data encompassing PII or other confidential attributes, machine unlearning offers a viable solution to decouple the model from such influences. By leveraging this approach, stakeholders can bolster user privacy, ensuring that the model's outputs remain devoid of any personal or sensitive traces.

% \paragraph{Eliminating outdated and incorrect information.}
% In our ever-evolving world, information has a shelf life. Today's veracious data can easily metamorphose into yesterday's obsolete knowledge. Consequently, LLMs, if rooted in antiquated data, can inadvertently disseminate outmoded or erroneous insights. Machine unlearning provides a mechanism to purge the vestiges of such dated datasets, enabling the model to refocus on contemporary and verifiable information. This is paramount in swiftly progressing domains like medicine or technology, where stale data can yield detrimental repercussions. By instituting periodic audits of the data underpinning LLMs and harnessing machine unlearning, these models can be kept abreast of current developments without the onus of exhaustive retraining.


% \paragraph{Addressing harmful and biased narratives.}
% It is an unfortunate reality that LLMs can mirror and amplify detrimental stereotypes, biases, or misinformation latent in their training datasets. Detecting and isolating the source of such harmful or prejudiced content within the model's outputs is a complex endeavor. However, once these detrimental data segments are identified, machine unlearning stands as a potent tool to mitigate or nullify their influence. By embracing this approach, one can curtail the perpetuation of damaging narratives and foster a more equitable and informed AI landscape.


% % \paragraph{Customized model deployment}
% % Different enterprises and institutions might want to deploy LLMs tailored to their specific needs or values. They might identify certain knowledge or biases in the general model that aren't aligned with their mission or ethos. Machine unlearning can be applied to customize these models by reducing the influence of undesirable data. Additionally, as models are deployed globally, there might be a need to ensure they are sensitive to local cultures and norms. Machine unlearning can help in removing or reducing influences that might be offensive or inappropriate in certain cultural contexts.

% \begin{table*}[!t]
% \centering
% \small
% \begin{tabular}{@{}l|c|c@{}}
% \toprule
%  & Unlearn Term & Retain Term \\
%   & $\sum_{w\in \mathcal{U}}\sum_{t=1}^{T} \log P_{M}(q_{t} | w_1, ..., w_{t-1}), q_t\sim Q_{w_t}$ & $\sum_{z\in \mathcal{R}}\sum_{t=1}^T\log P_{M}(z_t | z_1, ..., z_{t-1})$ \\ \midrule
% Gradient Ascend & $Q_{w_t} = \delta_{w_t} (q_t = w_t)$ and times $-1$ to the gradient & - \\
% Retain Fine-tune & - &  $\mathcal{R}=\mathcal{D}\setminus\mathcal{U}$  \\
% Random Label &  $Q_{w_t}= U(0,1)$ to be uniform distribution  & - \\
% Incompetent teacher &  $Q_{w_t}=P_{M_{\text{rand}}}(w_t|w_1, ..., w_{t-1})$ ,$M_{\text{rand}}$ is a rand init model  & -   \\
% Adversarial samples &  & -  \\
% % Reference Distribution &  &  \\
% Ours &  &  \\ \bottomrule
% \end{tabular}
% \caption{Summary of existing unlearning methods under our formulation}
% \end{table*}

